Analysis and Control of Input-Affine Dynamical Systems using Infinite-Dimensional Robust Counterparts

Input-affine dynamical systems often arise in control and modeling scenarios, such as the data-driven case when state-derivative observations are recorded under bounded noise. Common tasks in system analysis and control include optimal control, peak estimation, reachable set estimation, and maximum control invariant set estimation. Existing work poses these types of problems as infinite-dimensional linear programs in auxiliary functions with sum-of-squares tightenings. The bottleneck in most of these programs is the Lie derivative nonnegativity constraint posed over the time-state-control set. Decomposition techniques to improve tractability by eliminating the control variables include vertex decompositions (switching), or facial decompositions in the case where the polytopic set is a scaled box. This work extends the box-facial decomposition technique to allow for a robust-counterpart decomposition of semidefinite representable sets (e.g. polytopes, ellipsoids, and projections of spectahedra). These robust counterparts are proven to be equivalent to the original Lie constraint under mild compactness and regularity constraints. Efficacy is demonstrated under peak/distance/reachable set data-driven analysis problems and Region of Attraction maximizing control.

==> macros/jared_macro_ifac.tex <==
\usepackage{xcolor}
\usepackage{amsmath}
\usepackage{amssymb}
% \usepackage{amsthm}
\usepackage{mathtools}
\usepackage{subcaption}
\usepackage{hyperref}
% \usepackage[ruled]{algorithm2e}
\usepackage{mathrsfs}
\usepackage[printonlyused]{acronym}
\usepackage{tikz}
%revisions (changed text in this version vs. previous submission)
%initial->revised: blue
%revised->final:   purple
\newcommand{\rev}[1]{{\color{purple} #1}}
\newcommand{\old}[1]{{\color{teal} #1}}

%urgent (notes for authors)
\newcommand{\urg}[1]{{\color{red} #1}}
\newcommand{\MS}[1]{{\color{green} MS: #1}}

%Single Symbols
\newcommand{\E}{\mathbb{E}} 
\newcommand{\R}{\mathbb{R}} 
\newcommand{\K}{\mathbb{K}} 
\newcommand{\C}{\mathbb{C}} 
\newcommand{\N}{\mathbb{N}}
\newcommand{\D}{\mathbb{D}}
\newcommand{\Dc}{\mathcal{D}}
\newcommand{\Lie}{\mathcal{L}} 
\newcommand{\ks}{\mathcal{K}} 
\newcommand{\Z}{\mathbb{Z}}
\newcommand{\Zt}{\mathcal{Z}}
\newcommand{\s}{\mathcal{S}}
\newcommand{\M}{\mathbb{M}}

\newcommand{\A}{\mathcal{A}}
\newcommand{\0}{\mathbf{0}}
\newcommand{\1}{\mathbf{1}}
\newcommand{\psd}{\mathbb{S}}
\newcommand{\scL}{\mathscr{L}}
\newcommand{\vs}{\mathcal{V}}
\newcommand{\es}{\mathcal{E}}
\newcommand{\gs}{\mathcal{G}}
\newcommand{\bbm}{\mathbf{m}}

%Paired Commands
\DeclarePairedDelimiter{\abs}{\lvert}{\rvert}
\DeclarePairedDelimiter{\norm}{\lVert}{\rVert}
\DeclarePairedDelimiter{\ceil}{\lceil}{\rceil}
\DeclarePairedDelimiter{\Tr}{\textrm{Tr}(}{)}
\DeclarePairedDelimiter{\rank}{\textrm{rank}(}{)}
\DeclarePairedDelimiter{\diag}{\textrm{diag}(}{)}
\DeclarePairedDelimiter{\vvec}{\textrm{vec}(}{)}
\DeclarePairedDelimiter{\mmat}{\textrm{mat}(}{)}
\DeclarePairedDelimiterX{\inp}[2]{\langle}{\rangle}{#1, #2}
\DeclarePairedDelimiter{\supp}{\textrm{supp}(}{)}
\DeclarePairedDelimiter{\Mp}{\mathcal{M}_+(}{)}

%Operators and problems
\DeclareMathOperator*{\argmin}{arg\!\,min}
\DeclareMathOperator*{\argmax}{arg\!\,max}

%coloring
% \usepackage{xcolor}
\newcommand{\purp}[1]{\textcolor{purple}{#1}}


%fix coloring
\makeatletter
\renewcommand*{\@textcolor}[3]{
  \protect\leavevmode
  \begingroup
    \color#1{#2}#3%
  \endgroup
}
\makeatother

%theorem environment

% \newtheorem{thm}{Theorem}[section]
% \newtheorem{lem}[thm]{Lemma}
% \newtheorem{prop}[thm]{Proposition}
% \newtheorem{cor}{Corollary}
% \newtheorem{defn}{Definition}[section]
% \newtheorem{conj}{Conjecture}[section]
% \newtheorem{exmp}{Example}[section]
\newtheorem{rmk}{Remark}

\newcommand{\bpf}{\begin{pf}}
\newcommand{\epf}{\end{pf}}

==> macros/jared_macro_siads.tex <==
%Jared Miller's personal macros for acronyms and initialisms
\usepackage[printonlyused]{acronym}
\usepackage{xcolor}
\usepackage{amsmath}
% \usepackage{amsmath}
\usepackage{amssymb}
\usepackage{mathtools}
\usepackage{subcaption}
\usepackage{hyperref}
\hypersetup{colorlinks=true, linkcolor=black}
% \usepackage[ruled]{algorithm2e}
\usepackage{mathrsfs}
% \usepackage{tikz}

\newcommand{\rev}[1]{{\color{purple} #1}}
%urgent (notes for authors)
\newcommand{\urg}[1]{{\color{red} #1}}
\newcommand{\victor}[1]{{\color{blue} #1}}
\newcommand{\old}[1]{{\color{teal} #1}}
\newcommand{\MS}[1]{{\color{green} MS: #1}}
\definecolor{dkgreen}{rgb}{0,0.4,0}
\definecolor{dkred}{rgb}{0.7,0,0}
\newcommand{\MK}[1]{{\color{dkgreen}{#1}}}

%Single Symbols
\newcommand{\E}{\mathbb{E}} 
\newcommand{\R}{\mathbb{R}} 
\newcommand{\K}{\mathbb{K}} 
\newcommand{\C}{\mathbb{C}} 
\newcommand{\N}{\mathbb{N}}
\newcommand{\D}{\mathbb{D}}
\newcommand{\Dc}{\mathcal{D}}
\newcommand{\Lie}{\mathcal{L}} 
\newcommand{\ks}{\mathcal{K}} 
\newcommand{\Z}{\mathbb{Z}}
\newcommand{\Zt}{\mathcal{Z}}
\newcommand{\s}{\mathcal{S}}
\newcommand{\M}{\mathbb{M}}

\newcommand{\A}{\mathcal{A}}
\newcommand{\0}{\mathbf{0}}
\newcommand{\1}{\mathbf{1}}
\newcommand{\bm}{\mathbf{m}}
\newcommand{\psd}{\mathbb{S}}
\newcommand{\scL}{\mathscr{L}}
\newcommand{\vs}{\mathcal{V}}
\newcommand{\es}{\mathcal{E}}
\newcommand{\gs}{\mathcal{G}}

\newcommand{\dc}{\mathcal{D}}
\newcommand{\bbm}{\mathbf{m}}



%Paired Commands
\DeclarePairedDelimiter{\abs}{\lvert}{\rvert}
\DeclarePairedDelimiter{\norm}{\lVert}{\rVert}
\DeclarePairedDelimiter{\ceil}{\lceil}{\rceil}
\DeclarePairedDelimiter{\floor}{\lfloor}{\rfloor}
\DeclarePairedDelimiter{\Tr}{\textrm{Tr}(}{)}
\DeclarePairedDelimiter{\rank}{\textrm{rank}(}{)}
% \DeclarePairedDelimiter{\diag}{\textrm{diag}(}{)}
\DeclarePairedDelimiter{\vvec}{\textrm{vec}(}{)}
\DeclarePairedDelimiter{\mmat}{\textrm{mat}(}{)}
\DeclarePairedDelimiterX{\inp}[2]{\langle}{\rangle}{#1, #2}
\DeclarePairedDelimiter{\supp}{\textrm{supp}(}{)}
\DeclarePairedDelimiter{\Mp}{\mathcal{M}_+(}{)}

%Operators and problems
\DeclareMathOperator*{\argmin}{arg\!\,min}
\DeclareMathOperator*{\argmax}{arg\!\,max}

\DeclareMathOperator*{\find}{find}


\newcommand{\purp}[1]{\textcolor{purple}{#1}}

\newcommand{\fref}{\urg{[ref]}}

%theorem environment
% \usepackage{amsthm}
% \newtheorem{thm}{Theorem}[section]
% \newtheorem{lem}[thm]{Lemma}
% \newtheorem{prop}[thm]{Proposition}
% \newtheorem{prob}[thm]{Problem}
% \newtheorem{cor}{Corollary}
% \newtheorem{defn}{Definition}[section]
% \newtheorem{conj}{Conjecture}[section]
% \newtheorem{exmp}{Example}[section]
% \newtheorem{rmk}{Remark} 

% \newsiamremark{hypothesis}{Hypothesis}
% \crefname{hypothesis}{Hypothesis}{Hypotheses}
\newsiamthm{defn}{Definition}
\newsiamthm{thm}{Theorem}
\newsiamthm{lem}{Lemma}
\newsiamthm{cor}{Corollary}
\newsiamremark{rmk}{Remark}
\newsiamthm{prop}{Proposition}

\newcommand{\bpf}{\begin{proof}}
\newcommand{\epf}{\end{proof}}

==> robust_shared.tex <==
% SIAM Shared Information Template
% This is information that is shared between the main document and any
% supplement. If no supplement is required, then this information can
% be included directly in the main document.


% Packages and macros go here
\usepackage{lipsum}
\usepackage{amsfonts}
\usepackage{graphicx}
\usepackage{epstopdf}
\usepackage{algorithmic}
\ifpdf
  \DeclareGraphicsExtensions{.eps,.pdf,.png,.jpg}
\else
  \DeclareGraphicsExtensions{.eps}
\fi

% Prevent itemized lists from running into the left margin inside theorems and proofs
\usepackage{enumitem}
\setlist[enumerate]{leftmargin=.5in}
\setlist[itemize]{leftmargin=.5in}

% Add a serial/Oxford comma by default.
\newcommand{\creflastconjunction}{, and~}

% Used for creating new theorem and remark environments
\newsiamremark{remark}{Remark}
\newsiamremark{hypothesis}{Hypothesis}
\crefname{hypothesis}{Hypothesis}{Hypotheses}
\newsiamthm{claim}{Claim}

% Sets running headers as well as PDF title and authors
\headers{Parameterized Robust Counterparts for Systems Analysis}{J. Miller and M. Sznaier}

% Title. If the supplement option is on, then "Supplementary Material"
% is automatically inserted before the title.
\title{Analysis and Control of Input-Affine Dynamical Systems \\ using Parameterized Robust Counterparts\thanks{Submitted to the editors DATE.
\funding{J. Miller and M. Sznaier were partially supported by National Science Foundation (NSF) grants  CNS--1646121, CMMI--1638234, ECCS--1808381 and CNS--2038493,  and Air Force Office of Scientific Research (AFOSR) grant FA9550-19-1-0005. J. Miller was partially supported by the Swiss National Science Foundation under NCCR Automation, grant agreement 51NF40\_180545.
% J. Miller was partially supported by the Chateaubriand Fellowship.
This material is based upon research supported by the Chateaubriand Fellowship of the Office for Science \& Technology of the Embassy of France in the United States, and AFOSR's International Student Exchange Program (ISEP).}}}

% Authors: full names plus addresses.
\author{Jared Miller\thanks{Automatic Control Laboratory (IfA), Department of Information Technology and Electrical Engineering (D-ITET), ETH Z\"{u}rich, Physikstrasse 3, 8092, Z\"{u}rich, Switzerland (\email{jarmiller@control.ee.ethz.ch)}.}
\and Mario Sznaier\thanks{Robust Systems Lab,  ECE Department, Northeastern University, Boston, MA 02115
  (\email{msznaier@coe.neu.edu}).}}

\usepackage{amsopn}
\DeclareMathOperator{\diag}{diag}

\input{macros/jared_macro_siads}

%%% Local Variables: 
%%% mode:latex
%%% TeX-master: "ex_article"
%%% End: 


==> sections/reach_example.tex <==
\subsection{Reachable Set Example}

Figure \ref{fig:twist_reach} illustrates data-driven reachable set estimation on the Twist system from \eqref{eq:twist_dynamics} for a time horizon of $T=8$ by \ac{SOS} tightening to the Lie-robustified \eqref{eq:reach_cont}. The 100 observations from this system are pictured in Figure \ref{fig:twist_observed}, yielding a $L=9$-dimensional polytope with 34 non-redundant faces. As the order of tightening to program  increases from 3 to 4, the red region (level set of $\omega(x)$) tightens to the spiraling attractor region of the $T=8$ reachable set. The `volume' in the plot titles is not the true volume of the superlevel set $\{x \mid \phi(x) \geq 1\}$, but is instead the Lebesgue estimates $\int_X \phi(x) dx$.

 \begin{figure}[ht]
     \centering
     \begin{subfigure}[b]{0.48\linewidth}
         \centering
         \includegraphics[width=\linewidth]{fig/poly_3_lin_3_reach.png}
         \caption{\label{fig:twist_reach_3}Order 3 relaxation}
         
     \end{subfigure}
     \;
     \begin{subfigure}[b]{0.48\linewidth}
         \centering
         \includegraphics[width=\linewidth]{fig/poly_3_lin_4_reach.png}
         \caption{\label{fig:twist_reach_4}Order 4 relaxation}
     \end{subfigure}
      \caption{\label{fig:twist_reach}Reachable set estimation of twist \eqref{eq:twist_dynamics} system where $B^1$ is known and $B^3$ are unknown.}
\end{figure}



==> sections/roa_example.tex <==
\subsection{Region of Attraction Example}

This example of \ac{ROA} estimation will concentrate on a controlled version of the Flow dynamics from \eqref{eq:flow_w} under $L=6$ inputs
\begin{equation}
\label{eq:flow_controlled}
    \dot{x} = \textrm{Flow}(x) + \begin{bmatrix} w_1 + w_2 x_1 + w_3 x_2 \\
    w_4 + w_5 x_1 + w_6 x_2\end{bmatrix}
\end{equation}
obeying the polytopic input limits
\begin{equation}
    W = \left\{w \mid \begin{matrix}\norm{[w_1; w_4]}_\infty \leq 0.1, \ \norm{[w_2; w_3; w_5; w_6]}_\infty \leq 0.15 \\ \norm{[(w_1+w_2+w_3); (w_4+w_5+w_6)]}_\infty \leq 0.3 \end{matrix} \right\}.
\end{equation}

The circle $X_T = \{x \mid 0.1^2 - (x_1-0.5)^2 - (x_2-0.5)^2 \geq 0\}$ is the destination of the \ac{ROA} problem with a time horizon of $T = 5$ and a state space of $X = [-1.5, 1.5]^2$. The \ac{WSOS} tightening of the Lie-robustified Problem  \eqref{eq:roa_cont} yields bounds for the \ac{ROA} volume of $d^*_{2:6} =[9.000, \ 9.000, \ 6.717, \ 5.620, \ 5.187].$

The destination set $X_T$ is drawn in the black circle in the left subplot of Figure \ref{fig:flow_roa}. The white area is an outer approximation of the true \ac{ROA}, found as the superlevel set $\{x \mid \phi(x) \geq 1\}$ at order 6. The red area is the sublevel set $\{x \mid \phi(x) \leq 1\}$. The right subplot of Figure \ref{fig:flow_roa} draws the degree-12 polynomial function $\phi(x)$.


% The left plot of Figure \ref{fig:flow_roa} visualizes an outer approximation to the \ac{ROA} set (in white) that steers trajectore

% \urg{Need to implement \ac{ROA} and example}

\begin{figure}[ht]
         \centering
     \includegraphics[width=\linewidth]{fig/roa_flow_6_order_6.png}
      \caption{\label{fig:flow_roa} Order 6 \ac{ROA} for controlled Flow \eqref{eq:flow_controlled}}
\end{figure}


==> sections/sos_reduced.tex <==
\subsection{Sum-of-Squares Hierarchy}
\label{sec:moment_sos}

Let $p(x) \in \R[x]$ be a polynomial. The polynomial $p(x)$ is additionally \ac{SOS} if there exists a (non-unique) selection $q_i(x) \in \R[x]$ for $i=1..n_p$ with $n_p$ finite such that $p(x) = \sum_{i=1}^{n_p} q_i(x)^2$. Being \ac{SOS} is a certificate that $p(x)$ is nonnegative over the real numbers $x \in \R^n$, given that the square of each real number $q_i(x)^2$ is nonnegative. Each \ac{SOS} certificate may be expressed as a polynomial vector $v(x) \in \R[x]^s$ and a \ac{PSD} (\textit{Gram}) matrix $Q \in \psd_+^n$ such that $p(x) = v(x)^T Q v(x)$. The sum-factors $q(x) = \{q_i(x)\}_{i=1}^{n_p}$ may be recovered from $q(x) = Q^{\frac{1}{2}} v(x)$ for any matrix square root or factor $Q^{\frac{1}{2}}$. The cone of nonnegative polynomials over $\R^n$ is $\R[x]_+^n$, and its subcone of \ac{SOS} polynomials is $\Sigma[x]$. Verifying that a polynomial is nonnegative is generically NP-hard, but \ac{SOS} methods may be cast as \acp{SDP} and therefore solved to $\epsilon$-accuracy in polynomial time.  The set of $n$-variate $2d$-degree \ac{SOS} polynomials is equal to its corresponding supercone of nonnegative polynomials only when $n=1$ (univariate), $d=1$ (quadratic), or $(n=1, d=2)$ (bivariate quartic) \cite{hilbert1888darstellung}. Unfortunately, \ac{SOS} polynomials do not generally capture the full array of nonnegative polynomials. The ratio of volumes between these cones asymptotically decreases towards zero as $n \rightarrow \infty$ for each fixed degree $d > 2$ \cite{blekherman2006there}.

\Iac{BSA} set is the locus of finite-degree polynomial equality and inequality constraints, $\K= \{x \mid g_i(x) \geq 0, h_j(x) = 0 \ \forall i = 1..N_g, \ j=1..N_h\}$. \ac{BSA} sets are closed under intersection operations, but are not closed under unions and projections. The Putinar Positivestellensatz (Psatz) yields a sufficient condition for a polynomial $p(x) \in \R[x]$ to be positive $(p(x) > 0)$ over the \ac{BSA} set $\K$ 
\cite{putinar1993compact}, 
\begin{subequations}
\label{eq:putinar}
    \begin{align}
        & p(x) = \sigma_0(x) + \textstyle \sum_i {\sigma_i(x)g_i(x)} + \textstyle \sum_j {\phi_j(x) h_j}\\
        &\exists  \sigma_0(x) \in \Sigma[x], \quad \sigma(x) \in (\Sigma[x])^{N_g}, \quad \phi \in (\R[x])^{N_h}. \label{eq:putinar_variables}
    \end{align}
\end{subequations}

The \ac{WSOS} cone $\Sigma[\K]$ will denote the cone of polynomials $p(x)$ that admit a Putinar \eqref{eq:putinar} representation of positivity given the descriptor polynomials $g_i, h_j$ of $\K$.
\Iac{BSA} set satisfies an \textit{Archimedean} property if there exists a scalar $R \in (0, \infty)$ such that $R^2 - \norm{x}^2_2 \in \Sigma[\K]$. The Putinar psatz is a necessary and sufficient condition of positivity for Archimedean sets.

The moment-\ac{SOS} hierarchy is a computational method to produce a sequence of tightening outer approximations of infinite-dimensional \acp{LP} (in measures and functions) through the use of \acp{SDP}. The constrained polynomial optimization problem $P^* = \inf_{x \in \K} c(x)$ for $c(x) \in \R[x]$ over the Archimedean $\K$ may be expressed  as,
% as the primal-dual pair of \acp{LP},
\begin{align}
    P^* &= \sup_{\gamma \in \R} \ \gamma & & c(x) - \gamma \geq 0, \quad \forall x \in \K  \label{eq:poly_opt_k_nonneg}
\end{align}
The imposition $c(x) - \gamma \in \Sigma[\K]_{\leq 2d}$ (Putinar \eqref{eq:putinar} representation where all multipliers $\sigma_0, \sigma_i, \phi_j$ induce terms of degree at most $2d$) yields a bound $p^*_d \leq P^*$. Increasing the degree $d$ will produce a chain of lower bounds obeys $p^*_d \leq p^*_{d+1} \leq p^*_{d+2} \ldots$, and this sequence will converge with $\lim_{d \rightarrow \infty} p^*_d = P^*$ under the Archimedean assumption \cite{lasserre2009moments}.
% The dual problems to the putinar \acp{SDP} in \eqref{eq:poly_opt_k_nonneg} are \ac{LMI} relaxations of the measure program in \eqref{eq:poly_opt_k_meas}. The dual variable associated with the Gram matrix of $\sigma_0$ is the moment matrix of the measure $\mu$. \urg{how much detail should I add here?}


% Application of the Putinar psatz \eqref{eq:putinar} to the nonnegativity ......................................................................................................................

% \old{
% The constrained optimization problem of $P^* = \min_{x \in \K} c(x)$ may be expressed through a nonnegativity constraint as,
% \begin{subequations}
% \label{eq:poly_opt_k}
% \begin{align}
%     P^* &= \max_{\gamma \in \R} \ \gamma,\quad c(x) - \gamma \geq 0 & \forall x \in \K \label{eq:poly_opt_k_nonneg}
% \end{align}
% \end{subequations}
% M. Putinar introduced an algebraic certificate (Putinar Positivestellensatz) that is a necessary and sufficient condition for a function $p(x)$ to be positive over the Archimedean basic semialgebraic set $\K$ \cite{putinar1993compact},
% \begin{subequations}
% \label{eq:putinar}
%     \begin{align}
%         & p(x) = \sigma_0(x) + \textstyle \sum_i {\sigma_i(x)g_i(x)} + \textstyle \sum_j {\phi_j(x) h_j}\\
%         &\exists  \sigma_0(x) \in \Sigma[x], \qquad \sigma(x) \in (\Sigma[x])^{N_g}, \quad \phi \in (\R[x])^{N_h}. \label{eq:putinar_variables}
%     \end{align}
% \end{subequations}

% The degree-$d$ \ac{SOS} tightening of problem \eqref{eq:poly_opt_k} uses a bounded-degree Putinar Psatz in place of the nonnegativity constraint \eqref{eq:poly_opt_k_nonneg},
% \begin{subequations}
% \label{eq:poly_opt_sos}
% \begin{align}
%     d^*_d &= \sup \ \gamma 
%     \\
%     & c(x) - \gamma = \sigma_0(x) + \textstyle\sum_{i=1}^{N_c} {\sigma_i(x)g_i(x)} \\
%     & \sigma_i(x) \in \Sigma[x]_{2d} \quad \forall i = 0, \ldots, N_c
% \end{align}
% \end{subequations}
% Problem \eqref{eq:poly_opt_sos} is a \acf{SDP} in terms of elements of the finite-dimensional Gram matrices $Q_0 \ldots Q_{N_c}$ describing the Putinar multipliers $\sigma_0 \ldots \sigma_{N_c}$. The objective values between programs \eqref{eq:poly_opt_k} and \eqref{eq:poly_opt_sos} are related by $d^*_d \geq P^*$, and the chain of upper bounds obeys $d^*_d \geq d^*_{d+1} \geq d^*_{d+2} \ldots$ as the degree of the \ac{SOS} tightening increases \cite{lasserre2009moments}. When $\K$ is Archimedean, the objective value $d^*_d$ will converge to $P^*$ as the relaxation degree $d$ approaches $\infty$. The \ac{SOS} (moment-\ac{SOS}) hierarchy is the process of forming \acp{SDP} in increasing degree by replacing polynomial nonnegativity constraints by \ac{SOS} constraints.
% The size of a Gram matrix in $n$ variables and at degree $d$ is $N = \binom{n+d}{d}\approx n^d$. The per-iteration complexity of an Interior Point Method for solving an \ac{SDP} up to $\epsilon$-accuracy with an $N$-dimensional \ac{SDP} matrix and $M$ affine constraints is $O(N^3 M + N^2 M^2 + M^3)$ \cite{alizadeh1995interior}. This runtime is polynomial in $n$ for fixed $d$, and is combinatorial as $d$ increases in the \ac{SOS} hierarchy.
%  }
% Concepts in \ac{SOS} relaxations
% \urg{maybe bring this into nota


==> sections/summary.tex <==
% \urg{fix this when all content is in place}

This paper has the following layout: 
Section \ref{sec:preliminaries} provides an overview of preliminaries including notation, the analysis and control problems, robust counterparts, and \ac{SOS} theory.
% Section \ref{sec:prelim_robust} reviews the definition of \ac{SDR} sets, the concept of robust counterparts, and the notion of \acp{PMI}.
% Section \ref{sec:analysis_control_problem} poses the peak estimation, distance estimation, reachable set estimation, and \ac{BRS} maximization programs for systems of the form in \eqref{eq:disturbance_affine} with convex-bounded uncertainty $w$.
Section \ref{sec:lie_decomposed} splits the Lie derivative constraint over the \ac{SDR} uncertainty $W$ through the use of an parameterized robust counterpart. 
Section \ref{sec:robust_poly_approx} details \ac{SOS} programs for the robust counterparts. Section \ref{sec:discrete_time} applies parameterized robust counterparts to simplify problems with discrete-time dynamics.
% Section \ref{sec:poly_peak} applies the facial decomposition to peak estimation. \old{Section \ref{sec:reach} uses the facial decomposition for reachable set estimation and \ac{BRS} control problems.} 
Section \ref{sec:data_driven_background} reviews background of the polyhedral structure of consistency constraints induced by model structures and $L_\infty$-bounded noise processes. Section \ref{sec:robust_examples} presents examples of robust counterparts acting on all four problems. Section  \ref{sec:poly_conclusion} concludes the paper. 

% Appendix \ref{app:poly_robust_aux} extends a proof from \cite{fantuzzi2020bounding} that the auxiliary function for peak estimation under uncertainty may be approximated by a polynomial. 
% Appendix \ref{app:continuity_robust} contains a proof showing that multiplier functions associated with a certificate of Lie constraint nonnegativity may be chosen to be continuous. Appendix \ref{app:poly_robust_mult} shows that the multiplier functions may be approximated by polynomials.
% Appendix \ref{app:analysis_control_problem} lists infinite-dimensional \acp{LP} for distance estimation, reachable set estimation, and \ac{ROA} maximization.
% Appendix \ref{app:integral_cost} applies robust counterparts to Lie constraints that possess integral terms (running costs).
%  Appendix \ref{app:robust_duality} discusses dual measure \acp{LP} to the developed infinite-dimensional robust counterparts and applies a moment-based  scheme from \cite{majumdar2014convex, korda2014convex} to recover polynomial controller laws. 

% \old{Section \ref{sec:preliminaries} provides an overview of preliminaries including notation, \ac{SOS} theory, and \ac{SOS} applications for analysis and control problems. Section \ref{sec:lie_decomposed} splits the Lie derivative constraint over the polytopic uncertainty $W$ through the use of a facial decomposition. Section \ref{sec:poly_peak} applies the facial decomposition to peak estimation. Section \ref{sec:reach} uses the facial decomposition for reachable set estimation and \ac{BRS} control problems. Section \ref{sec:data_driven_background} reviews background of the polyhedral structure of consistency constraints induced by model structures and $L_\infty$-bounded noise processes. Section \ref{sec:poly_peak_example} presents examples of facial decompositions acting on all three problems. The paper is concluded in section \ref{sec:poly_conclusion}. Appendix \ref{app:continuity} contains a proof that multiplier functions associated with a certificate of Lie constraint nonnegativity may be chosen to be continuous. Appendix \ref{app:poly} shows that the multiplier functions may be approximated by polynomials.
% }
